Quantum Gravitational Corrections to Electromagnetism And Backreaction

This dissertation examines the impact of quantum gravity on electromagnetism and its backreaction, using perturbative general relativity as an effective field theory. Our analysis involves quantum-correcting Maxwell's equations to obtain a gauge-independent, real, and causal effective field equation that describes quantum gravitational effects on electromagnetism. Additionally, we present a perturbative mechanism through which quantum gravity induces a dimension six coupling between a massive scalar and electromagnetism. To investigate the effects of electromagnetism on the gravitational sector, we derive an exact, dimensionally regulated, Fourier mode sum for the Lorentz gauge propagator of a massive photon on an arbitrary cosmological background supported by a scalar inflaton. This allows us to calculate the effective potential induced by photons. Finally, we use a similar Fourier mode sum for a time-dependent mass to study the effective force on the inflaton 0-mode and its impact on reheating.

==> abbreviations.tex <==
\singlespacing
\begin{tabular}{l p{5in}} 
%if the terms in the first column are longer than 1.4 inches reduce the number 5 appropriately
$\sum$ & Denotes the summation of a series of terms\\
\\%This adds the single space between definitions (required)
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.\\

\end{tabular}
\doublespacing


==> abstractFile.tex <==
This dissertation examines the impact of quantum gravity on electromagnetism and its backreaction, using perturbative general relativity as an effective field theory. Our analysis involves quantum-correcting Maxwell's equations to obtain a gauge-independent, real, and causal effective field equation that describes quantum gravitational effects on electromagnetism. Additionally, we present a perturbative mechanism through which quantum gravity induces a dimension six coupling between a massive scalar and electromagnetism.

To investigate the effects of electromagnetism on the gravitational sector, we derive an exact, dimensionally regulated, Fourier mode sum for the Lorentz gauge propagator of a massive photon on an arbitrary cosmological background supported by a scalar inflaton. This allows us to calculate the effective potential induced by photons. Finally, we use a similar Fourier mode sum for a time-dependent mass to study the effective force on the inflaton 0-mode and its impact on reheating.

==> acknowledgementsFile.tex <==
I would like to express my sincere gratitude to my advisor, Prof. Richard P. Woodard, for his invaluable guidance, unwavering support, and patience throughout my doctoral journey. His vast knowledge and experience have not only aided me in my academic pursuits but also enriched my personal life. Prof. Woodard has set an exceptionally high standard for mentorship, which I aspire to emulate.

My heartfelt gratitude also extends to my collaborator, Prof. Shun-Pe Miao, and to the distinguished members of my supervisory committee, Profs. Laura Blecha, David Groisser, Pierre Sikivie, Charles Thorn, and Bernard Whiting, for their invaluable input and constant encouragement. Moreover, I am deeply appreciative of the physics department’s entire faculty and staff, including the exceptional Ms. Pam Marlin, whose administrative acumen proved indispensable.

Furthermore, I would like to acknowledge the support and encouragement of my parents Ganga Bahadur and Chhabimaya, my wife Rojina, my sisters Samikshya and Sarita, and my in-laws Gopal and Shakti. Without their understanding and support this journey would have been much more challenging. Lastly but not leastly, I want to thank Richelle, my tiny little daughter who made the final year much more joyful.

==> biographyFile.tex <==
Jhapa, Nepal is where Sanjib was born and raised. After completing middle school, he moved to the bustling capital of Kathmandu, where he earned his bachelor's and master's degrees in physics from Tribhuvan University.

Overcoming challenges, Sanjib relocated to Gainesville, Florida in 2017 to pursue his academic goals at the University of Florida. There, he focused on his doctoral studies in physics, working under the guidance of Professor Richard Woodard, a renowned physicist known for his research on the intersection of particle physics and cosmology.

Keenly focused on his studies, Sanjib made remarkable progress in his research despite the challenges of adjusting to life in a new country. In April of 2023, he successfully defended his dissertation and earned his PhD in Physics in the summer of 2023.

Encouraged by the love and support of his wife Rojina and their daughter Richelle, Sanjib remained steadfast in his commitment to both his family and his studies, serving as an inspiration to others who aspire to achieve their dreams through hard work and perseverance.

==> dedicationFile.tex <==
To all the giants upon whose broad shoulders I have stood, for this creation is cobbled together from various bits and blobs

==> editorAndAuthorRemarks.tex <==
If you don't see any blue or red type under this line, then you almost certainly need to include the optional ``editMode" to the document class. Thus your document class (first line) should read \verb|\documentclass[editMode]{ufdissertation}|

\authorRemark{Test! This is a remark written by the author, to themselves, for review purposes. It will be suppressed unless editMode is used in the class options.}

\editorRemark{This is an editor's remark, written by an editor in-line so that they can write into the content itself with something easy to see. But the remark will be suppressed unless editMode is used in the class options.

To get this remark to go away, simply remove ``editMode" from the documentclass options at the top of the user's tex-file. This also removes the blue Author Remarks.}

